Logging Requirement for Continuous Auditing of Responsible Machine Learning-based Applications

Machine learning (ML) is increasingly applied across industries to automate decision-making, but concerns about ethical and legal compliance remain due to limited transparency, fairness, and accountability. Monitoring through logging a long-standing practice in traditional software offers a potential means for auditing ML applications, as logs provide traceable records of system behavior useful for debugging, performance analysis, and continuous auditing. systematically auditing models for compliance or accountability. The findings underscore the need for enhanced logging practices and tooling that systematically integrate responsible AI metrics. Such practices would support the development of auditable, transparent, and ethically responsible ML systems, aligning with growing regulatory requirements and societal expectations. By highlighting specific deficiencies and opportunities, this work provides actionable guidance for both practitioners and tool developers seeking to strengthen the accountability and trustworthiness of ML applications.

==> declaration.tex <==
\textbf{Conflicts of interests/Competing interests:} The authors declare that they have no known competing financial interests or personal relationships that could have appeared to influence the work reported in this paper.

\noindent\textbf{Data availability statement:} The datasets generated during and/or analysed during the current study are available in the [foalem] repository, [\url{https://shorturl.at/FLg9z}].

% Declarations

% Funding 
% No funding was received for conducting this study.

% Conflicts of interest/Competing interests
% The authors have no relevant financial or non-financial interests to disclose.

% Availability of data and material
% The datasets generated during and/or analysed during the current study are available in the Github repository, https://github.com/senseconcordia/TestLoggingPractice.

% Code availability
% Code for data cleaning and analysis is provided as part of the replication package. It is available at https://github.com/senseconcordia/TestLoggingPractice.

% \begin{titlepage}
%     Declarations

% % Funding 
% % No funding was received for conducting this study.

% Conflicts of interest/Competing interests
% The authors declare that they have no known competing financial interests or personal relationships that could have appeared to influence the work reported in this paper.


% Code availability
% The datasets generated during and/or analysed during the current study are available in the [foalem] repository, [\url{https://shorturl.at/FLg9z}].
% \end{titlepage}
